Hierarchical Time Series Forecasting with Bayesian Modeling

We encounter time series data in many domains such as finance, physics, business, and weather. One of the main tasks of time series analysis, one that helps to take informed decisions under uncertainty, is forecasting. Time series are often hierarchically structured, e.g., a company sales might be broken down into different regions, and each region into different stores. In some cases the number of series in the hierarchy is too big to fit in a single model to produce forecasts in relevant time, and a decentralized approach is beneficial. One way to do this is to train independent forecasting models for each series and for some summary statistics series implied by the hierarchy (e.g. the sum of all series) and to pass those models to a reconciliation algorithm to improve those forecasts by sharing information between the series. In this work we focus on the reconciliation step, and propose a method to do so from a Bayesian perspective - Bayesian forecast reconciliation. We also define the common case of linear Gaussian reconciliation, where the forecasts are Gaussian and the hierarchy has linear structure, and show that we can compute reconciliation in closed form. We evaluate these methods on synthetic and real data sets, and compare them to other work in this field.

==> content/empirical_evaluation/empirical_copy.tex <==

\section{Data Sets}
\label{sec:experiments:data_sets}
\addcontentsline{tocheb}{section}{\protect\numberline{\secnumforhebrewtoc}{מערכי נתונים}}

\subsection{Synthetic Data Set - Experiment A}
\label{subsec:experiments:data_sets:synthetic_a}
\addcontentsline{tocheb}{subsection}{\protect\numberline{\subsecnumforhebrewtoc}{מערך נתונים סינטטיים - ניסוי א}}
\begin{figure}	
	\centering
	\resizebox{0.5\linewidth}{!}{\input{content/empirical_evaluation/synthetic.tex}}
	\caption{The synthetic data set in~\ref{subsec:experiments:data_sets:synthetic_a}. The four systems $\{x^{(n)}\}_{n=1}^4$ are connected to the same parent $u$.}
	\label{fig:experiments:data_sets:synthetic_a}
\end{figure}
The first experiment include a synthetic dataset consisting of a hierarchy of 4 series all connected to same parent, as shown in Figure~\ref{fig:experiments:data_sets:synthetic_a}.
Each series is a sine wave, corrupted by noise. The observations are the first period of the sine wave and the task is to predict the second cycle.

Observations for each series marked as $y^{(i)}_t$, and the future (hidden) states marked $x^{(i)}_t$ for the bottom series and $u_t$ for the sum of the series. A bold symbol, $\pmb{x}^{(n)}$, is a vector of all time steps, and $\pmb{x}_t$, is a vector of all series in time step $t$.\\
Data was created: 
\begin{align}
    y_t^{(n)} &= \sin (t) + \epsilon_t^{(n)}, \quad t \in [0, 2\pi), \quad \epsilon_t^{(n)} \sim \mathcal{N}(0, \sigma_{\epsilon}) \quad \forall n=\{1,2,3,4\}\\
    x_t^{(n)} &= \sin (t) + \epsilon_t^{(n)}, \quad t \in [2\pi, 4\pi], \quad \epsilon_t^{(n)} \sim \mathcal{N}(0, \sigma_{\epsilon}) \quad \forall n=\{1,2,3,4\}
\end{align}
In the different experiments on this data set we experimented with these noise levels: $\sigma_{\epsilon} \in \{0, 0.1, 0.2, 0.5, 1, 2, 5\}$.\\
The sum of series is given by:
\begin{equation}
    u_t = f(\pmb{x}_t) = \sum_{i=1}^4 x^{(i)}_t
\end{equation}
\textbf{Base forecasts} where created by fitting a GP (\ref{subsec:background:forecasting:gpr}) to the observations $\pmb{y}^{(n)}$ and are parameterized by $\{\Theta^{(n)}\}_{n=1}^4$ for each series $\{\pmb{x}^{(n)}\}_{n=1}^4$ and $\Eta$ for $\pmb{u}$:
\begin{equation}
\label{eqn:experiments:data_sets:synthetic_a:base_forecasts}
    \hat{\pmb{x}}^{(n)} \equiv \pmb{x}^{(n)} | \Theta^{(n)} \sim \mathcal{GP}^{(n)} \quad \forall n=\{1,2,3,4\}, \quad \pmb{u} | \Eta \sim \mathcal{GP}
\end{equation}
The GP's are set with a scaled periodic kernel (see~\ref{eqn:background:gpr:periodic_kernel}). The period length hyperparameter $p$ is assumed to be known and fixed at $2\pi$, which is a common case in many applications where the seasonality is known.

\textbf{Reconciliation} for each time step is performed independently, so the reconciler actually gets the marginalised prediction for time step $t$:
$$\hat{x}_t^{(n)} \equiv x_t^{(n)} | \Theta_t^{(n)} \sim \mathcal{N}_t^{(n)} \quad \forall n=\{1,2,3,4\}, \quad u_t | \Eta_t \sim \mathcal{N}_t$$
A visualization of the data set and the base forecasts can be seen in Figure~\ref{fig:experiments:data_sets:synthetic_a}.
\begin{figure}
    \includegraphics[scale=0.5, width=14cm]{content/empirical_evaluation/synthetic_data2_cropped.png}
	\centering
	\caption{Example of data set and its base forecasts for $\sigma_{\epsilon}=\{0.1,0.2,0.5\}$. Black x's denote train data (observations $\pmb{y}^{(n)}$), green x's denote test data ($\pmb{x}^{(n)}$), blue line and shaded blue area denote the mean and 95\% confidence interval of the base forecasts, respectively.}
	\label{fig:experiments:data_sets:synthetic_a}
\end{figure}

\subsection{Synthetic Data Set - Experiment B}
\label{subsec:experiments:data_sets:synthetic_b}
\addcontentsline{tocheb}{subsection}{\protect\numberline{\subsecnumforhebrewtoc}{מערך נתונים סינטטיים - ניסוי ב}}
This setting is the exact same setting as in \ref{subsec:experiments:data_sets:synthetic_a}, with the only difference that the base forecasts themselves, for the bottom level only, where "shifted" for each series by some random noise. So instead of Equation~\ref{eqn:experiments:data_sets:synthetic_a:base_forecasts} we now have:
\begin{equation}
\label{eqn:experiments:data_sets:synthetic_b:base_forecasts}
    \hat{\pmb{x}}^{(n)}_{B} = \hat{\pmb{x}}^{(n)}_{A} + \zeta^{(n)}, \quad \zeta^{(n)} \sim \mathcal{N}(0, 1) \quad \forall n=\{1,2,3,4\}, \quad \pmb{u} | \Eta \sim \mathcal{GP}
\end{equation}
where $\hat{\pmb{x}}^{(n)}_{A}, \hat{\pmb{x}}^{(n)}_{B}$ are the base forecasts in Experiments A and B respectively.
\textbf{Reconciliation} is done the same as in \ref{subsec:experiments:data_sets:synthetic_a}.
A visualization of the data set and the "shifted" base forecasts can be seen in Figure~\ref{fig:experiments:data_sets:synthetic_b}.
\begin{figure}
    \includegraphics[scale=0.5, width=14cm]{content/empirical_evaluation/synthetic_data_b_cropped.png}
	\centering
	\caption{Example of data set and its "shifted" base forecasts for $\sigma_{\epsilon}=\{0.1,0.2,0.5\}$. Black x's denote train data (observations $\pmb{y}^{(n)}$), green x's denote test data ($\pmb{x}^{(n)}$), blue line and shaded blue area denote the mean and 95\% confidence interval of the base forecasts, respectively.}
	\label{fig:experiments:data_sets:synthetic_b}
\end{figure}

\subsection{Real Data Set}
\label{subsec:experiments:data_sets:real}
\addcontentsline{tocheb}{subsection}{\protect\numberline{\subsecnumforhebrewtoc}{מערך נתונים אמיתיים}}
\begin{figure}
	\centering
    \includegraphics[scale=0.5, width=14cm]{content/empirical_evaluation/real_data.png}
	\caption{The first level of the hierarchy of the dataset. Top graph: the number of visitors by month to each of the seven states of Australia. Bottom graph: The sum of the series in the top graph.}
	\label{fig:experiments:data_sets:real}
\end{figure}
The real data set we tested on is a data set consisted of the number of tourists who entered Australia on a monthly basis, by their reason of entrance (Holiday, Visitor, Business, Other), between 1998 to 2016. On the bottom level the data set contains 304 time series referring to Australia's 76 regions and 4 reasons of entrance. The data is then aggregated to 27 macro zones and then to 7 states on the upper level. We chose to test the 7 series of the total tourists entered to each state. A visualization of the data set is shown in Figure~\ref{fig:experiments:data_sets:real}.
\textbf{Base forecasts} where created using the same methodology of the synthetic data set (see~\ref{subsec:experiments:data_sets:synthetic_a}), with the only difference that the period length parameter was constrained to $p \in [12-0.1, 12+0.1]$ and that we added an RBF kernel (see~\ref{eqn:background:gpr:rbf_kernel}).
\textbf{Reconciliation} here also performed independently as in \ref{subsec:experiments:data_sets:synthetic_a}, and got the same marginalised prediction for time step $t$.
The main change here regarding train and test data, is that we are splitting the data set into train and test in different point in each simulation we will perform, i.e., we will perform 50 simulation, each with 60 time steps (5 years) as train data and 24 time steps (2 years) as test data, starting from the first period.


\section{Metrics}
\label{sec:experiments:metrics}
\addcontentsline{tocheb}{section}{\protect\numberline{\secnumforhebrewtoc}{מדדי ביצועים}}
In each experiment we will compare two reconcilation methods. The first method is the one presented in~\ref{subsec:theory:model:linear-model} we will call \textit{ET Reconciler}, the second method is the \textit{LG} method presented in \cite{hier-bayes-paper} and we will call it \textit{Bayes Paper LG Reconciler}. Each reconciliation method tested should produce a reconciled probability $\tilde{\mathcal{D}}_t$ for each time step $t$.
For each reconciliation method we are computing the \textit{Negative Log Predictive Density} (NLPD):
\begin{equation}
    \text{NLPD} = \frac{1}{T} \sum_t -\log{p_{\tilde{\mathcal{D}}_t}(\pmb{x}_t)}
\end{equation}
i.e., the average, over the time steps, of the negative log of the true values $\pmb{x}$ under the reconciled probability density function $\tilde{\mathcal{D}}$.
As mentioned in all Data Sets in~\ref{sec:experiments:data_sets}, we will test each data set produced with noise levels: $\sigma_{\epsilon} \in \{0, 0.1, 0.2, 0.5, 1, 2, 5\}$.
For each data set in~\ref{sec:experiments:data_sets} and each noise level $\sigma_{\epsilon}$, we will perform $N=50$ simulations and compute the \textit{NLPD}. We will report the mean, the standard error of the mean (denoted as SEM) and the standard deviation (denoted as SD) of the \textit{NLPD}s of those $N$ simulations for each reconciliation method (and for the base forecasts as a benchmark).


\section{Results}\label{sec:experiments:results}
\addcontentsline{tocheb}{section}{\protect\numberline{\secnumforhebrewtoc}{תוצאות}}

\subsection{Results - Synthetic Data Set - Experiment A}
\label{subsec:results:data_sets:synthetic_a}
\addcontentsline{tocheb}{subsection}{\protect\numberline{\subsecnumforhebrewtoc}{תוצאות - מערך נתונים סינטטיים - ניסוי א}}

\begin{table}[]
    \centering
    \begin{tabular}{|ll|r|r|r|}
    \hline
    {} & {} & {Base Forecast} & {Bayes Paper LG Reconciler} & {ET Reconciler} \\
    \hline
    \multirow[c]{3}{*}{$\sigma_{\epsilon}=0$} & \textit{mean} & -15.73 & \textbf{-15.85} & -15.04 \\
    & \textit{SEM} & 0.00 & 0.00 & 0.00 \\
    & \textit{SD} & 0.00 & 0.00 & 0.00 \\
    \hline
    \multirow[c]{3}{*}{$\sigma_{\epsilon}=0.1$} & \textit{mean} & 2.13 & 2.88 & \textbf{0.26} \\
    & \textit{SEM} & 0.52 & 0.59 & 0.35 \\
    & \textit{SD} & 3.67 & 4.18 & 2.48 \\
    \hline
    \multirow[c]{3}{*}{$\sigma_{\epsilon}=0.2$} & \textit{mean} & 3.77 & 4.37 & \textbf{2.43} \\
    & \textit{SEM} & 0.47 & 0.53 & 0.33 \\
    & \textit{SD} & 3.35 & 3.78 & 2.31 \\
    \hline
    \multirow[c]{3}{*}{$\sigma_{\epsilon}=0.5$} & \textit{mean} & 6.61 & 7.17 & \textbf{5.73} \\
    & \textit{SEM} & 0.37 & 0.42 & 0.27 \\
    & \textit{SD} & 2.59 & 2.95 & 1.91 \\
    \hline
    \multirow[c]{3}{*}{$\sigma_{\epsilon}=1$} & \textit{mean} & 44.38 & 48.55 & \textbf{39.92} \\
    & \textit{SEM} & 21.82 & 24.00 & 19.32 \\
    & \textit{SD} & 154.31 & 169.71 & 136.61 \\
    \hline
    \multirow[c]{3}{*}{$\sigma_{\epsilon}=2$} & \textit{mean} & 139.82 & 163.48 & \textbf{134.89} \\
    & \textit{SEM} & 109.48 & 127.55 & 106.00 \\
    & \textit{SD} & 774.13 & 901.95 & 749.51 \\
    \hline
    \multirow[c]{3}{*}{$\sigma_{\epsilon}=5$} & \textit{mean} & 29.84 & 34.14 & \textbf{29.74} \\
    & \textit{SEM} & 9.64 & 11.68 & 9.43 \\
    & \textit{SD} & 68.16 & 82.60 & 66.71 \\
    \hline
    \end{tabular}
\caption{Results for the experiment on Data Set~\ref{subsec:experiments:data_sets:synthetic_a}.}
\label{tab:results:data_sets:synthetic_a}
\end{table}
In Table~\ref{tab:results:data_sets:synthetic_a} are the results for experiment on Data Set~\ref{subsec:results:data_sets:synthetic_a}.

The first takeaway is that the algorithm proposed in~\ref{pro:lg} works, i.e., the \textit{ET Reconciler} improves the \textit{NLPD} score compared to the base forecasts (except for the case where $\sigma_{\epsilon} = 0$ which we will explain about in a bit).

Another takeaway from looking at the results is that we can notice that except for when the data was generated with $\sigma_{\epsilon} = 0$, \textit{ET Reconciler} always outperformed \textit{Bayes Paper LG Reconciler}. Here is some intuition for why.

The base forecasts were generated using GPs (see~\ref{eqn:experiments:data_sets:synthetic_a:base_forecasts}), and the kernels of a GP have an additive property, i.e., the sum of the four periodic kernels of the bottom time series is also a periodic kernel. So, we expect that the mean of the base forecasts for the upper time series will be close to the sum of the means of the base forecasts for the bottom time series, and in the notations of~\ref{subsec:theory:model:linear-model}, we expect that $A \pmb{\mu}_{\theta}$ and $\pmb{\mu}_{\eta}$ will be close.
In both reconciliation methods (\textit{ET Reconciler} and \textit{Bayes Paper LG Reconciler}) there is a mechanism (see $\mu_{LG}$ in Proposition~\ref{pro:lg:mu-lg} and Section 3.1 in~\cite{hier-bayes-paper}) to correct the means of the base forecasts if there is a difference between the mean of the upper series and the means of the bottom series after being passed through the mapping $f(\pmb{x})$, in this data set it is a summation.
Since we used GPs to generate the forecasts there isn't a big difference between the means and both reconciliation methods report a similar mean.

So the difference between the reconcilers must come from the covariance.

What happens is that \textit{ET Reconciler} adds to the covariance of the base predictions, the difference between the covariance of the prediction for the upper series and the transformed (after the linear mapping) covariance of the prediction for the bottom series (see $\Sigma_{LG}$ in Proposition~\ref{pro:lg:sigma-lg}), wheres in \textit{Bayes Paper LG Reconciler} they always reduce the covariance of the reconciled predictions (see Section 3.1 in~\cite{hier-bayes-paper}).
This property of the reconcilers make \textit{ET Reconciler} to enlarge it's total variance, whereas \textit{Bayes Paper LG Reconciler} reduce it's total variance, and as the data set is getting more "noisy", i.e., $\sigma_{\epsilon}$ gets larger (up to a certain level) the reconciler with the larger total variance gets a better \textit{NLPD} score.

As for the experiment where the data set has no noise ($\sigma_{\epsilon} = 0$), what happens is that the base forecasts are quite accurate to begin with and the mean of them is precise, so in order to make the \textit{NLPD} score better one needs to reduce the variance, and that is why this is the only case that \textit{Bayes Paper LG Reconciler} gets a better score. This is of course a very extreme case where the base forecasts are accurate and there is no noise in the data set. Also, the magnitude of improvement of the \textit{NLPD} is very small compare to other settings of $\sigma_{\epsilon}$.


\subsection{Results - Synthetic Data Set - Experiment B}
\label{subsec:results:data_sets:synthetic_b}
\addcontentsline{tocheb}{subsection}{\protect\numberline{\subsecnumforhebrewtoc}{תוצאות - מערך נתונים סינטטיים - ניסוי ב}}

\begin{table}[]
    \centering
    \begin{tabular}{|ll|r|r|r|}
    \hline
    {} & {} & {Base Forecast} & {Bayes Paper LG Reconciler} & {ET Reconciler} \\
    \hline
    \multirow[c]{3}{*}{$\sigma_{\epsilon}=0$} & \textit{mean} & 15947.89 & 15191.35 & \textbf{12166.44} \\
    & \textit{SEM} & 1727.36 & 1675.84 & 1549.79 \\
    & \textit{SD} & 12214.29 & 11849.97 & 10958.69 \\
    \hline
    \multirow[c]{3}{*}{$\sigma_{\epsilon}=0.1$} & \textit{mean} & 367.63 & 348.50 & \textbf{265.19} \\
    & \textit{SEM} & 46.69 & 44.55 & 38.77 \\
    & \textit{SD} & 330.15 & 315.02 & 274.13 \\
    \hline
    \multirow[c]{3}{*}{$\sigma_{\epsilon}=0.2$} & \textit{mean} & 109.28 & 103.90 & \textbf{79.01} \\
    & \textit{SEM} & 10.64 & 9.83 & 7.75 \\
    & \textit{SD} & 75.21 & 69.51 & 54.83 \\
    \hline
    \multirow[c]{3}{*}{$\sigma_{\epsilon}=0.5$} & \textit{mean} & 20.82 & 20.59 & \textbf{16.75} \\
    & \textit{SEM} & 1.86 & 1.80 & 1.60 \\
    & \textit{SD} & 13.15 & 12.70 & 11.30 \\
    \hline
    \multirow[c]{3}{*}{$\sigma_{\epsilon}=1$} & \textit{mean} & 52.74 & 58.21 & \textbf{43.30} \\
    & \textit{SEM} & 23.05 & 27.23 & 18.19 \\
    & \textit{SD} & 163.00 & 192.53 & 128.64 \\
    \hline
    \multirow[c]{3}{*}{$\sigma_{\epsilon}=2$} & \textit{mean} & 164.91 & 177.92 & \textbf{153.76} \\
    & \textit{SEM} & 102.91 & 112.67 & 98.58 \\
    & \textit{SD} & 727.67 & 796.71 & 697.07 \\
    \hline
    \multirow[c]{3}{*}{$\sigma_{\epsilon}=5$} & \textit{mean} & 107.73 & 119.53 & \textbf{106.10} \\
    & \textit{SEM} & 41.73 & 47.53 & 42.00 \\
    & \textit{SD} & 295.09 & 336.06 & 296.97 \\
    \hline
    \end{tabular}
\caption{Results for the experiment on Data Set~\ref{subsec:experiments:data_sets:synthetic_b}.}
\label{tab:results:data_sets:synthetic_b}
\end{table}

In Table~\ref{tab:results:data_sets:synthetic_b} are the results for experiment on Data Set~\ref{subsec:results:data_sets:synthetic_b}.

As a reminder, for the second experiment on the synthetic data set, we added noise to the base forecasts themselves by adding a constant to the mean of those forecasts of the bottom series only.

Here we can notice that again for all settings of $\sigma_{\epsilon}$ \textit{ET Reconciler} outperforms \textit{Bayes Paper LG Reconciler} and even for when $\sigma_{\epsilon} = 0$. This happens here because for all settings the reconcilers must also change the mean of the base forecasts, and also the covariance, so the fact that for $\sigma_{\epsilon} = 0$ there is no noise doesn't effect the improvement of the \textit{NLPD} compared to the base forecasts.
As in the results of the previous experiment~\ref{tab:results:data_sets:synthetic_a}, the \textit{NLPD} improves up to a certain level of noise in the data. Also to notice that here even for a very large noise ($\sigma_{\epsilon} = 5$), \textit{ET Reconciler} improves the \textit{NLPD} whereas \textit{Bayes Paper LG Reconciler} doesn't.


\subsection{Results - Real Data Set}
\label{subsec:results:data_sets:real}
\addcontentsline{tocheb}{subsection}{\protect\numberline{\subsecnumforhebrewtoc}{תוצאות - מערך נתונים אמיתיים}}

\begin{table}[]
    \centering
    \begin{tabular}{|l|r|r|r|}
    \hline
    {} & {\textit{mean}} & {\textit{SEM}} & 
    {\textit{SD}} \\
    \hline
    Base Forecast & 60.56 & 0.41 & 2.88 \\
    \hline
    Bayes Paper LG Reconciler & 61.19 & 0.41 & 2.87 \\
    \hline
    ET Reconciler & \textbf{59.35} & 0.42 & 2.99 \\
    \hline
    \end{tabular}
\caption{Results for the experiment on Data Set~\ref{subsec:experiments:data_sets:real}.}
\label{tab:results:data_sets:real}
\end{table}

In Table~\ref{tab:results:data_sets:real} are the results for experiment on Data Set~\ref{subsec:results:data_sets:real}.

Here we can see that our proposed method works for a real data set also.

The results here are telling a similar story to what happened in~\ref{subsec:results:data_sets:synthetic_a}, since the data set is pretty noisy but the sum of the base forecasts generated for the bottom series have similar mean to the base forecasts of the sum of those series, and the property of enlarging the covariance of \textit{ET Reconciler}, as opposed to decreasing the covariance in \textit{Bayes Paper LG Reconciler}, results in an improvement of the \textit{NLPD} in favor of our proposed method.

==> main_pages/title_page.tex <==
\begin{titlepage}
    \begin{center}
        % \vspace*{1cm}
        
        \includegraphics[width=0.1\textwidth]{Main_pages/bgu.png}\\
        Ben-Gurion University of the Negev\\
        The Faculty of Natural Sciences\\
        The Department of Computer Science
        
        \vspace{1cm}
        
        {\Large \thesistitle}
        
        \vspace{0.5cm}
        
        Thesis submitted in partial fulfillment of the requirements\\for the Master of Sciences degree
        
        \vspace{0.5cm}
        
        \thesisauthorname
        
        \vspace{0.5cm}
        
        Under the supervision of \thesissupervisername
        
        \vspace{0.5cm}
        
        \begin{flushleft}
        Signature of student: \( \rule{3cm}{0.15mm} \) \hfill Date: \( \rule{3cm}{0.15mm} \)\\
        Signature of supervisor: \( \rule{3cm}{0.15mm} \) \hfill Date: \( \rule{3cm}{0.15mm} \)\\
        Signature of supervisor: \( \rule{3cm}{0.15mm} \) \hfill Date: \( \rule{3cm}{0.15mm} \)\\
        Signature of chairperson of the\\committee for graduate studies: \( \rule{3cm}{0.15mm} \) \hfill Date: \( \rule{3cm}{0.15mm} \)
        \end{flushleft}
        
        \vfill
        
        \thesismonth \quad \thesisyear
    \end{center}
\end{titlepage}
